Trade-Offs Between Fairness and Privacy in Language Modeling

Protecting privacy in contemporary NLP models is gaining in importance. So does the need to mitigate social biases of such models. But can we have both at the same time? Existing research suggests that privacy preservation comes at the price of worsening biases in classification tasks. In this paper, we explore the extent to which this tradeoff really holds when we incorporate both privacy preservation and de-biasing techniques into training text generation models. How does improving the model along one dimension affect the other dimension as well as the utility of the model? We conduct an extensive set of experiments that include bias detection, privacy attacks, language modeling, and performance on downstream tasks.

==> draft.tex <==
To avoid the leakage of sensitive data through language models, methods have been introduced to protect the privacy of the data. This includes Differential Privacy (DP; \citeauthor{dwork2014algorithmic} (\citeyear{dwork2014algorithmic}), which has been used in many domains. \citeauthor{abadi2016deep} (\citeyear{abadi2016deep}) has introduced DP Stochastic Gradient Descent (DP-SGD) to implement DP directly in the training of language models. The disadvantage of it though is high computational and memory overhead which \citeauthor{yu2021large} (\citeyear{yu2021large}) tried to tackle with their approach of parameterized gradient perturbation (RGP). They create a low-dimensional projection of the gradient of each layers weight matrix and then introduce privacy by clipping and noising these low-dimensional gradients.
\citeauthor{shi2021selective} (\citeyear{shi2021selective}) further elaborated the influence of privacy on the utility of a model and emphasized the importance of understanding the trade-off between privacy and utility. To improve utility they introduced the approach of selective-DP (S-DP) for RNN-based language models and thereby allowed different attributes in the data to have different privacy levels. 
S-DP got further extended by the approach of the \textit{fine-tuning twice privacy mechanism} for large transformer models. S-DP here is obtained by finetuning the model first with redacted in-domain data and then again with the original and private in-domain data (\cite{shi2022just}). 
